Data-Driven Control of Positive Linear Systems using Linear Programming

This paper presents a linear-programming based algorithm to perform data-driven stabilizing control of linear positive systems. A set of state-input-transition observations is collected up to magnitude-bounded noise. A state feedback controller and dual linear copositive Lyapunov function are created such that the set of all data-consistent plants is contained within the set of all stabilized systems. This containment is certified through the use of the Extended Farkas Lemma and solved via Linear Programming. Sign patterns and sparsity structure for the controller may be imposed using linear constraints. The complexity of this algorithm scales in a polynomial manner with the number of states and inputs. Effectiveness is demonstrated on example systems.

==> sections/abstract.tex <==
\begin{abstract}
\label{sec:abstract}
This paper presents a linear-programming based algorithm to perform data-driven stabilizing control of linear positive systems. A set of state-input-transition observations is collected up to magnitude-bounded noise. A state feedback controller and dual linear copositive Lyapunov function are created such that the set of all data-consistent plants is contained within the set of all stabilized systems. This containment is certified through the use of the Extended Farkas Lemma and solved via Linear Programming. Sign patterns and sparsity structure for the controller may be imposed using linear constraints. The complexity of this algorithm scales in a polynomial manner with the number of states and inputs. Effectiveness is demonstrated on example systems.

\end{abstract}

==> sections/acknowledgements.tex <==
\section{Acknowledgements}

\urg{Optional acknowledgements. 
% Siami if we talk to him about this?
}

==> sections/conclusion.tex <==
\section{Conclusion}

\label{sec:conclusion}

This paper presented an LP-based algorithm (Theorem \ref{thm:poly_contain_lp}) to perform data-driven stabilizing control of positive linear systems. The state-feedback controller $K$ stabilizes all possible systems in the $L_\infty$-norm bounded consistency set $\Sigma_\dc$, as certified by a common \ac{DLCLF} function $V(x) = \max(x./v)$  and the Extended Farkas Lemma. There is no conservativeness in such a design: Equation \eqref{eq:lp_stab} will find a controller iff there exists such a linear copositive Lyapunov function across all consistent systems. This framework can also be used to perform data-driven worst-case peak-to-peak gain minimization using Equation \eqref{eq:p2p}.

Future work includes imposing forms of consistency sets for the noise (e.g. elementwise L2 norm bounds, semidefinite energy-based noise bounds for $\bw$). Other avenues include 
creating controllers in the switched or linear-parameter-varying setting, and extending this method towards Monotone systems. 

% An alternative  approach involves using polynomial-optimization hierarchies for copositive matrices by allowing for common quadratic copositive Lyapunov functions \cite{parrilo2000structured}. 

%\urg{Conclude the paper. Summarize the problem and important findings. Add some extensions and future work.}

%An extended Arxiv version of this paper is available at \urg{[Arxiv link goes here] what will the arxiv version have that this work does not?}.


==> sections/contributions.tex <==

The contributions of this work are:
\begin{itemize}
    \item \Iac{LP} that performs data-driven positive-stabilizing control for all systems consistent with observed data.
    \item A tabulation of computational complexity required to solve this \ac{LP}.
    \item An extension of this \ac{LP} towards worst-case peak-to-peak gain minimizing control.
\end{itemize}

==> sections/extensions.tex <==
\section*{Extensions}

\urg{To be saved for journal paper

\begin{itemize}
    \item Switching (Same controller, subsystem controllers, LPV, choosing the switching sequence)
    \item Other noise models ($L_2$, Semidefinite/energy)
    \item Bounded input control, ROA
    \item EIV control for positive systems based on the methods of \cite{miller2022eiv_short, miller2022eivarx}
\end{itemize}

I have implemented same-controller, subsystem-controllers, and LPV of 1. I need to find a good working example of the Lyapunov-Metzler inequalities in discrete-time to choose the switching sequence.

I have a rough example for 2 (L2-bounded noise), which should be enough for the case study. This uses Yalmip's robust optimization module.

I don't yet have code for bounded-input control.

EIV for positive system should go in its own paper (ACC 2024?). Much of the math is the same ($n^2 + n$ Psatz constraints for a single system in state-space, $n_p + n_c + 2$ constraints for SISO control), but there are some additional considerations and linear constraints that may be added in when the underlying plant is Metzler/Nonnegative.

}
% % \subsection{Structured Control}
% % \urg{Sign-based information on the values of $K$. Linear constraints to impose that $K_{jk} [\geq, =, \leq] 0$.}

% \subsection{Other Noise Models}
% \urg{$L_2$ noise, Semidefinite/energy noise. We can use robust counterparts and everything will be non-conservative and tight.}
% \begin{rmk}
% \urg{we might not need to write the discrepency matrix}

% Other noise models include elementwise constraints on $\norm{w}_2^2$ or energy constraints such that $P - \bw \bw^T$ is positive semidefinite for some known positive definite $P$ matrix.
% \end{rmk}
% \subsection{Switching}

% \urg{This could be in a separate journal paper. There is a large amount of material on copositive Lypapunov functions for  switching positive systems.

% We can talk about three basic models of switching:
% \begin{itemize}
%     \item Common Controller with different $(A, B)$
%     \item Individual-system controller and (possibly) Lyapunov Function with different $(A, B)$
%     \item LPVA (different $A$, same $B$) system: common Lypunov function with gain-scheduled controller.
% \end{itemize}


% }

==> sections/summary.tex <==

This paper has the following structure: 
Section \ref{sec:preliminaries} reviews the preliminaries of notation, positive systems, copositive Lyapunov functions, and the Extended Farkas Lemma.
Section \ref{sec:stab} presents \iac{LP} to perform data-driven stabilizing control of positive systems. Section \ref{sec:peaktopeak} extends this \ac{LP} framework to yield controllers that minimize the worst-case peak-to-peak gain between an external input and a controlled output.
Section \ref{sec:examples} demonstrates effectiveness of these methods on stabilizing and worst-case-optimal control of example systems.
Section \ref{sec:conclusion} concludes the paper.

==> sections_arxiv/diff_dlclf.tex <==
\subsubsection{Different DLCLF, Different Controller}

This task will assume that \eqref{eq:switched_traj} is \iac{DTS} the controller has access to the switching sequence. Furthermore, the switching transitions of \eqref{eq:switched_traj} are described by a directed graph $\gs$ in which the vertices $\vs$ are the subsystems $1..N_s$. The edges $\es$ describe possible transitions: given a pair of systems $(i, j) \in (1..N_s)^2$, the edge $(i, j) \in \es$ if the switching sequence can obey $S(t)=i$ and $S(t+1)=j$. We note that self-loops are allowed in $\es$, and that discrete-time dwell-time constraints may be implemented by inflating the number of subsystems.

Each subsystem $s$ will possess \iac{DLCLF} with parameter $v_s > 0$ and a controller matrix $K_s$.
\begin{thm}
\Iac{DTS} \eqref{eq:switched_traj} that obeys the switching constraints $\gs$ is positive-stabilized by the switching-dependent feedback controller $u(t) = K_{S(t)} x(t)$ if there exists a tolerance $\eta > 0$,  vectors $v_s > 0$, matrices $X_s = \diag{v}$ and $Y_s \in \R^{m_s \times n}$  for all $s\in 1..N_s$ if for each arc $(i, j) \in \es$ the following equation holds,
\begin{align}
\label{eq:lyap_arc}
    v_i - (A_{j} X_j + B_j Y_j)\1_n - \eta\1_n \in \R_{\geq 0}^n.
\end{align}
The subsystem controller gains may be recovered $K_s = Y_s X_s^{-1}$ for each $s=1..N_s$.
\end{thm}
\begin{proof}
Let $V_s(x) = \max(x./v_s)$ be the \ac{DLCLF} for each subsystem $s\in1..N_s$. Equation \ref{eq:lyap_arc} represents the statement that
\begin{align}
        \forall (i,j) &\in \es: \qquad V_i(x) - V_j(x) > 0 
\end{align}

\end{proof}
